Towards a machine learning pipeline in reduced order modelling for inverse problems: neural networks for boundary parametrization, dimensionality reduction and solution manifold approximation

In this work, we propose a model order reduction framework to deal with inverse problems in a non-intrusive setting. Inverse problems, especially in a partial differential equation context, require a huge computational load due to the iterative optimization process. To accelerate such a procedure, we apply a numerical pipeline that involves artificial neural networks to parametrize the boundary conditions of the problem in hand, compress the dimensionality of the (full-order) snapshots, and approximate the parametric solution manifold. It derives a general framework capable to provide an ad-hoc parametrization of the inlet boundary and quickly converges to the optimal solution thanks to model order reduction. We present in this contribution the results obtained by applying such methods to two different CFD test cases.

==> sections/notation.tex <==
%\begin{multicols}{2}
\small
\subsubsection*{Abbreviations}
\begin{tabular}{ll}
\cfd{} & Computational Fluid Dynamics \\
\rom{} & Reduced Order Model \\
PDE & Partial Differential Equation \\
\podec{} & Proper Orthogonal Decomposition \\
\nn{} & Artificial Neural Network \\
\autoe{} & AutoEncoder  \\
\rbf{} & Radial Basis Function
\end{tabular}
\subsubsection*{Symbols}
\begin{tabular}{ll}
$\sigma$ & activation function in \nn{} \\
$M$ & number of snapshots in \rom{} \\
$p$ & number of parameters used in \rom{} \\
$P$ & number of degrees of freedom for the velocity field \\
$L$ & latent dimension \\
$(\boldsymbol{\varphi})_{i=1}^M$ & velocity \podec{} modes \\
$\Vert \cdot \Vert$ & norm in $L^2$
\end{tabular}
%\end{multicols}
